ePBR: Extended PBR Materials in Image Synthesis

Realistic indoor or outdoor image synthesis is a core challenge in computer vision and graphics. The learning-based approach is easy to use but lacks physical consistency, while traditional Physically Based Rendering (PBR) offers high realism but is computationally expensive. Intrinsic image representation offers a well-balanced trade-off, decomposing images into fundamental components (intrinsic channels) such as geometry, materials, and illumination for controllable synthesis. However, existing PBR materials struggle with complex surface models, particularly high-specular and transparent surfaces. In this work, we extend intrinsic image representations to incorporate both reflection and transmission properties, enabling the synthesis of transparent materials such as glass and windows. We propose an explicit intrinsic compositing framework that provides deterministic, interpretable image synthesis. With the Extended PBR (ePBR) Materials, we can effectively edit the materials with precise controls.

==> fig/compose2.tex <==
\begin{figure*}[h]
    \centering
    \setlength{\resLen}{0.1\linewidth}
    \addtolength{\tabcolsep}{-7pt}
    \begin{tabular}{cccc@{\hskip -2pt}c@{\hskip -2pt}c@{\hskip -2pt}c}
        \begin{overpic}[width=\resLen]{iv/5/normal.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/5/albedo.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/5/roughness.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/5/irradiance.png} 
        \end{overpic} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/5/im_rgbx.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/5/im_ours.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/5/im.png} 
            \end{overpic}} \\[-4pt]
        \begin{overpic}[width=\resLen]{iv/5/depth.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/5/metallic.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/5/transparency.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/5/reflect_ssrt.png} 
        \end{overpic}
        \\[-2pt]
        \begin{overpic}[width=\resLen]{iv/6/normal.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/6/albedo.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/6/roughness.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/6/irradiance.png} 
        \end{overpic} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/6/im_rgbx.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/6/im_ours.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/6/im.png} 
            \end{overpic}} \\[-4pt]
        \begin{overpic}[width=\resLen]{iv/6/depth.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/6/metallic.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/6/transparency.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/6/reflect_ssrt.png} 
        \end{overpic}
        \\[-2pt]
        \begin{overpic}[width=\resLen]{iv/7/normal.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/7/albedo.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/7/roughness.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/7/irradiance.png} 
        \end{overpic} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/7/im_rgbx.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/7/im_ours.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/7/im.png} 
            \end{overpic}} \\[-4pt]
        \begin{overpic}[width=\resLen]{iv/7/depth.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/7/metallic.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/7/transparency.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/7/reflect_ssrt.png} 
        \end{overpic}
        \\[-2pt]
        \begin{overpic}[width=\resLen]{iv/8/normal.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/8/albedo.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/8/roughness.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/8/irradiance.png} 
        \end{overpic} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/8/im_rgbx.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/8/im_ours.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/8/im.png} 
            \end{overpic}} \\[-4pt]
        \begin{overpic}[width=\resLen]{iv/8/depth.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/8/metallic.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/8/transparency.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/8/reflect_ssrt.png} 
        \end{overpic}
        \\[-2pt]
        \begin{overpic}[width=\resLen]{iv/9/normal.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/9/albedo.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/9/roughness.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/9/irradiance.png} 
        \end{overpic} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/9/im_rgbx.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/9/im_ours.png} 
            \end{overpic}} &
        \multirow{2}{*}[28pt]{
            \begin{overpic}[width=2\resLen]{iv/9/im.png} 
            \end{overpic}} \\[-4pt]
        \begin{overpic}[width=\resLen]{iv/9/depth.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/9/metallic.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/9/transparency.png} 
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/9/reflect_ssrt.png} 
        \end{overpic}
        \\ 
        \multicolumn{4}{c}{Intrinsic representation} & RGB$\leftrightarrow$X & Ours & Reference
    \end{tabular}
    \caption{
        Image composition.
    }
    \label{fig:compose2}
\end{figure*}


==> fig/edit.tex <==
\begin{figure}
    \centering
    \setlength{\resLen}{0.5\linewidth}
    \addtolength{\tabcolsep}{-5pt}
    \begin{tabular}{cc}
        \includegraphics[width=\resLen]{iv/7/im.png} &
        \includegraphics[width=\resLen]{iv/7/im.png} 
        \\
        \includegraphics[width=\resLen]{iv/5/im.png} &
        \includegraphics[width=\resLen]{iv/5/im.png} 
    \end{tabular}
    \caption{\label{fig:edit}
        Image editing. \todo{}{Not done yet, two examples, comparing to other methods}
    }
\end{figure}

==> fig/insert.tex <==
\begin{figure}
    \centering
    \setlength{\resLen}{0.5\linewidth}
    \addtolength{\tabcolsep}{-5pt}
    \begin{tabular}{cc}
       \includegraphics[width=\resLen]{bedroom/ori.png} &
       \includegraphics[width=\resLen]{bedroom/trans.png} 
       \\
       \includegraphics[width=\resLen]{bedroom/ori.png} &
       \includegraphics[width=\resLen]{bedroom/trans.png} 
    \end{tabular}
    \caption{\label{fig:insert}
        Object insert. \todo{}{Not done yet, two examples, comparing to other methods}
    }
\end{figure}

==> fig/intrinsic.tex <==
\begin{figure}
    \centering
    \setlength{\resLen}{0.33\linewidth}
    \addtolength{\tabcolsep}{-6pt}
    \begin{tabular}{ccc}
        \begin{overpic}[width=\resLen]{intrinsic/normal.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $\N$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{intrinsic/depth.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $\D$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{intrinsic/albedo.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $\A$}}
        \end{overpic}
        \\
        \begin{overpic}[width=\resLen]{intrinsic/rough.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $\R$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{intrinsic/metal.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $\M$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{intrinsic/st.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $\T$}}
        \end{overpic}
        \\
        \begin{overpic}[width=\resLen]{intrinsic/irradiance.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $\E$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{intrinsic/reflect.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $\Amr$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{intrinsic/image.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $\Abg$}}
        \end{overpic}
    \end{tabular}
    \caption{
        Intrinsic channels.
    }
    \label{fig:intrinsic}
\end{figure}


==> fig/lpips.tex <==
\begin{figure*}[ht]
    \centering
    \setlength{\resLen}{0.185\linewidth}
    \addtolength{\tabcolsep}{-4pt}
    \begin{tabular}{cccccc}
        \raisebox{30pt}{\rotatebox[origin=c]{90}{RGB$\leftrightarrow$X}} &  
        \begin{overpic}[width=\resLen]{iv/0/lpips_rgbx_0.493.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.493$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/2/lpips_rgbx_0.360.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.360$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/4/lpips_rgbx_0.372.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.372$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/5/lpips_rgbx_0.387.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.387$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/7/lpips_rgbx_0.327.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.327$}}
        \end{overpic}
        \\
        \raisebox{30pt}{\rotatebox[origin=c]{90}{Ours}} &  
        \begin{overpic}[width=\resLen]{iv/0/lpips_ours_0.414.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.414$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/2/lpips_ours_0.271.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.271$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/4/lpips_ours_0.360.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.360$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/5/lpips_ours_0.336.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.336$}}
        \end{overpic} &
        \begin{overpic}[width=\resLen]{iv/7/lpips_ours_0.304.png} 
            \put(0, 3){\scriptsize \colorbox{white}{\color{black} $0.304$}}
        \end{overpic}
        \\
        & (a) & (b) & (c) & (d) & (e)
    \end{tabular}
    \caption{
        \textbf{LPIPS error maps} for \cref{fig:compose1}. Top row is the LPIPS between RGB$\leftrightarrow$X and Reference; bottom row is the LPIPS between Ours and Reference. The numbers at the corner of each error maps indicate the mean LPIPS error of the image.
    }
    \label{fig:lpips}
\end{figure*}


==> fig/principled.tex <==
\begin{figure*}[t]
    \centering
    \setlength{\resLen}{0.22\linewidth}
    \addtolength{\tabcolsep}{-5pt}
    \begin{tabular}{cccccc}
        % \multicolumn{2}{c}{Metallic} & \multicolumn{2}{c}{Roughness}
        \includegraphics[width=\resLen]{main/m0.png} &
        \includegraphics[width=\resLen]{main/m2.png} &
        \includegraphics[width=\resLen]{main/m4.png} &
        \includegraphics[width=\resLen]{main/m6.png} &
        \includegraphics[width=\resLen]{main/m8.png} &
        \includegraphics[width=\resLen]{main/m10.png} 
        \\
        \multicolumn{6}{c}{0 <------ Metallic ------> 1}
        \\
        \includegraphics[width=\resLen]{main/r0.png} &
        \includegraphics[width=\resLen]{main/r1.png} &
        \includegraphics[width=\resLen]{main/r2.png} &
        \includegraphics[width=\resLen]{main/r3.png} &
        \includegraphics[width=\resLen]{main/r4.png} &
        \includegraphics[width=\resLen]{main/r5.png} 
        \\
        \includegraphics[width=\resLen]{main/t0.png} &
        \includegraphics[width=\resLen]{main/t2.png} &
        \includegraphics[width=\resLen]{main/t4.png} &
        \includegraphics[width=\resLen]{main/t6.png} &
        \includegraphics[width=\resLen]{main/t8.png} &
        \includegraphics[width=\resLen]{main/t10.png} 
        \\
    \end{tabular}
    \caption{
        Principled BRDF evaluation
    }
    \label{fig:main}
\end{figure*}

==> fig/principledthin.tex <==
\begin{figure}[h]
    \centering
    \setlength{\resLen}{0.22\linewidth}
    \addtolength{\tabcolsep}{-5pt}
    \begin{tabular}{cccc}
        \multicolumn{2}{c}{Metallic} & \multicolumn{2}{c}{Roughness}
        \\
        \includegraphics[width=\resLen]{principledthin/ours/st/1.png} &
        \includegraphics[width=\resLen]{principledthin/ref/st/1.png} &
        \includegraphics[width=\resLen]{principledthin/ours/rough/1.png} &
        \includegraphics[width=\resLen]{principledthin/ref/rough/1.png} 
        \\
        \includegraphics[width=\resLen]{principledthin/ours/st/2.png} &
        \includegraphics[width=\resLen]{principledthin/ref/st/2.png} &
        \includegraphics[width=\resLen]{principledthin/ours/rough/2.png} &
        \includegraphics[width=\resLen]{principledthin/ref/rough/2.png} 
        \\
        % \includegraphics[width=\resLen]{principledthin/ours/st/3.png} &
        % \includegraphics[width=\resLen]{principledthin/ref/st/3.png} &
        % \includegraphics[width=\resLen]{principledthin/ours/rough/3.png} &
        % \includegraphics[width=\resLen]{principledthin/ref/rough/3.png} 
        % \\
        \includegraphics[width=\resLen]{principledthin/ours/st/4.png} &
        \includegraphics[width=\resLen]{principledthin/ref/st/4.png} &
        \includegraphics[width=\resLen]{principledthin/ours/rough/4.png} &
        \includegraphics[width=\resLen]{principledthin/ref/rough/4.png} 
        \\
        \includegraphics[width=\resLen]{principledthin/ours/st/5.png} &
        \includegraphics[width=\resLen]{principledthin/ref/st/5.png} &
        \includegraphics[width=\resLen]{principledthin/ours/rough/5.png} &
        \includegraphics[width=\resLen]{principledthin/ref/rough/5.png} 
        \\
        Ours & Ref & Ours & Ref
    \end{tabular}
    \caption{\label{fig:principledthin}
        Principled BSDF evaluation
    }
\end{figure}

==> fig/teaser.tex <==
\begin{center}
    \setlength{\resLen}{100pt}
    \begin{tabular}{c}
        \begin{overpic}[width=\linewidth]{teaser/teaser.png}
            \put(5, -2){\small \bfseries \color{black} (a) Rough dielectric}
            \put(27, -2){\small \bfseries \color{black} (b) Mirror}
            \put(47, -2){\small \bfseries \color{black} (c) Screen}
            \put(67, -2){\small \bfseries \color{black} (d) Glass}
            \put(80, -2){\small \bfseries \color{black} (e) Colored glass/plastic}
        \end{overpic}
    \end{tabular}
    \vspace{1em}
    \captionof{figure}{
        Rendering examples of different types of materials. \todo{}{Teaser will be updated.}
    }
    \label{fig:teaser}
\end{center}
